A lightweight PUF-based authentication protocol

Lightweight authentication is essential for resource-constrained Internet-of-Things (IoT). Implementable with low resource and operable with low power, Physical Unclonable Functions (PUFs) have the potential as hardware primitives for implementing lightweight authentication protocols. The arbiter PUF (APUF) is probably the most lightweight strong PUF capable of generating exponentially many challenge-response pairs (CRPs), a desirable property for authentication protocols, but APUF is severely weak against modeling attacks. Efforts on PUF design have led to many PUFs of higher resistance to modeling attacks and also higher area overhead. There are also substantial efforts on protocol development, some leverage PUFs' strength in fighting modeling attacks, and some others employ carefully designed protocol techniques to obfuscate either the challenges or the responses with modest increase of area overhead for some or increased operations for some others. To attain both low resource footprint and high modeling attack resistance, in this paper we propose a co-design of PUF and protocol, where the PUF consists of an APUF and a zero-transistor interface that obfuscates the true challenge bits fed to the PUF. The obfuscated PUF possesses rigorously proven potential and experimentally supported performance against modeling attacks when a condition is met, and the protocol provides the condition required by the PUF and leverages the PUF's modeling resistance to arrive at low resource overhead and high operational simplicity, enabling lightweight authentications while resisting modeling attacks.

==> protocol_fig.tex <==
\begin{table}[!ht]
\centering
\caption{Proposed mutual authentication protocol flow.}
\begin{tabularx}{\columnwidth}{X|X}
\hline
\textbf{Device $i$} & \textbf{Server} \\
\hline
& $\text{do while } (c_s \text{ used for } ID_i)$ \\
$c_s \leftarrow \text{TRNG}(n/2)$ & \\
$clr \leftarrow 0$ & $c_s \leftarrow$ \\
$S \leftarrow '1'$ & $ID_i || c_d \rightarrow$ \\
$c \leftarrow \text{PRNG}(c_s)$ & Abort if $ID_i$ is invalid or $c_d$ has been used \\
$c_d \leftarrow \text{SPUF}^{\prime}(c)$ & \\
& Add $c_d$ into used $c_d$ list of $ID_i$ \\
 & $c \leftarrow \text{PRNG}(c_s || c_d)$ \\
 & $r_1 || r_2 || r_3 \leftarrow \text{SPUF}_\text{model}(c)$ \\
 & $P_{\text{os}} \leftarrow \text{TRNG}(L - 1)$ \\
 & $h_1 \leftarrow P_{\text{os}} \oplus r_1$ \\
 & $h_2 \leftarrow P_{\text{os}} \oplus r_2$ \\
$h_1 || h_3 \leftarrow$ & $h_3 \leftarrow r_1 \oplus r_3$ \\
$c \leftarrow \text{PRNG}(c_s || c_d)$ & \\
$S \leftarrow '0'$ & \\
$\tilde{r_1} || \tilde{r_2} || \tilde{r_3} \leftarrow \text{SPUF}(c)$ & \\
$h_3 \leftarrow \tilde{r_1} \oplus \tilde{r_3}$ & \\
If FHD$(h_3, h_3) < \tau,$ & $\tilde{h_2} \rightarrow$ \\
\ \ \ $P_{\text{os}} \leftarrow h_1 \oplus \tilde{r_1}$ & If $d = \text{FHD}(\tilde{h_2}, h_2) > \tau,$ abort \\
\ \ \ load $P_{\text{os}}$ into register $P$ & \\
\ \ \ $h_2 \leftarrow P_{\text{os}} \oplus \tilde{r_2}$ & \\
Else & \\
\ \ \ $S \leftarrow '1'$, & \\
\ \ \ $h_2 \leftarrow \text{SPUF}^{\prime}(c)$ & \\
$clr \leftarrow 0, S \leftarrow '1'$ & \\
\hline
\end{tabularx}
\label{tab:protocol_flow}
\end{table}
